AI in Software Engineering: Perceived Roles and Their Impact on Adoption

This paper investigates how developers conceptualize AI-powered Development Tools and how these role attributions influence technology acceptance. Through qualitative analysis of 38 interviews and a quantitative survey with 102 participants, we identify two primary Mental Models: AI as an inanimate tool and AI as a human-like teammate. Factor analysis further groups AI roles into Support Roles (e.g., assistant, reference guide) and Expert Roles (e.g., advisor, problem solver). We find that assigning multiple roles to AI correlates positively with Perceived Usefulness and Perceived Ease of Use, indicating that diverse conceptualizations enhance AI adoption. These insights suggest that AI4SE tools should accommodate varying user expectations through adaptive design strategies that align with different Mental Models.

==> Table_1.tex <==
\begin{table}[ht]
\centering
\small
\begin{tabular}{lcc}
\toprule
Role & Factor1 & Factor2 \\
\midrule
As an assistant         &       & 0.657 \\
As a tool               &       & 0.495 \\
As a reference guide    &       & 0.506 \\
As a content generator  &       &       \\
As a problem solver     & 0.599 &       \\
As a collaborator       &       &       \\
As a senior colleague   &       &       \\
As a junior colleague   &       & 0.470 \\
As a teacher            &       &       \\
As an advisor           & 0.662 &       \\
As a reviewer           & 0.691 &       \\
As a copilot            &       &       \\
As a companion          &       &       \\
\bottomrule
\end{tabular}
\caption{Factor loadings (only values $\geq$ 0.4 are displayed).}
\label{tab:factor_loadings}
\end{table}
